Improving Model-based Genetic Programming for Symbolic Regression of Small Expressions

The Gene-pool Optimal Mixing Evolutionary Algorithm (GOMEA) is a model-based EA framework that has been shown to perform well in several domains, including Genetic Programming (GP). Differently from traditional EAs where variation acts blindly, GOMEA learns a model of interdependencies within the genotype, i.e., the linkage, to estimate what patterns to propagate. In this article, we study the role of Linkage Learning (LL) performed by GOMEA in Symbolic Regression (SR). We show that the non-uniformity in the distribution of the genotype in GP populations negatively biases LL, and propose a method to correct for this. We also propose approaches to improve LL when ephemeral random constants are used. Furthermore, we adapt a scheme of interleaving runs to alleviate the burden of tuning the population size, a crucial parameter for LL, to SR. We run experiments on 10 real-world datasets, enforcing a strict limitation on solution size, to enable interpretability. We find that the new LL method outperforms the standard one, and that GOMEA outperforms both traditional and semantic GP. We also find that the small solutions evolved by GOMEA are competitive with tuned decision trees, making GOMEA a promising new approach to SR.

==> results_test3.tex <==
\begin{table*}
\caption{Median test NMSE with $l \leq 15$, details as in Table~\ref{tab:validation3}.}\label{tab:test3}
\centering
\setlength{\tabcolsep}{0.01em}
\scalebox{0.7}{
\begin{tabular}{lScScSccScScSccScScSccScScScSc}
\toprule
 & \multicolumn{6}{c}{$n_\text{pop}=1000$} & \ssW{}\ssW{} & \multicolumn{6}{c}{IMS $g=4$} & \ssW{}\ssW{} & \multicolumn{6}{c}{IMS $g=6$} & \ssW{}\ssW{} & \multicolumn{8}{c}{IMS $g=8$} \\
 
Dataset \ssW{}& \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO}
& \multicolumn{2}{c}{DTR}\\
\midrule

Air & 
%fixpop
\multicolumn{2}{c}{\ssW{}26.4\ssW{}}& 
\ssW{}30.3 &\wtC{cbScarlet}{}&
\ssW{}37.2 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}26.1\ssW{}}&
\ssW{}23.7 &\btC{cbScarlet}{}&
\ssW{}37.4 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}25.1\ssW{}}&
\ssW{}25.3 &\ssW{}&
\ssW{}39.5 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}25.0\ssW{}}&
\ssW{}26.1 &\ssW{}&
\ssW{}39.1 &\wtC{cbScarlet}{}&
% DTR
\ssW{}31.2 &\wtC{cbScarlet}{} 
\\


Bos & 
%fixpop
\multicolumn{2}{c}{\ssW{}20.8\ssW{}}& 
\ssW{}20.9 &\wtC{cbScarlet}{}&
\ssW{}26.4 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}18.8\ssW{}}&
\ssW{}21.3&\wtC{cbScarlet}{}&
\ssW{}22.8&\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}20.4\ssW{}}&
\ssW{}21.5 &\wtC{cbScarlet}{}&
\ssW{}22.7 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}20.0\ssW{}}&
\ssW{}21.4 &\wtC{cbScarlet}{}&
\ssW{}24.4 &\wtC{cbScarlet}{}&
% DTR
\ssW{}25.5 &\wtC{cbScarlet}{} 
\\

Con & 
%fixpop
\multicolumn{2}{c}{\ssW{}17.4\ssW{}}& 
\ssW{}17.7 &\wtC{cbScarlet}{}&
\ssW{}21.6 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}16.9\ssW{}}&
\ssW{}17.1&\wtC{cbScarlet}{}&
\ssW{}21.6 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}16.6\ssW{}}&
\ssW{}16.9&\ssW{}&
\ssW{}21.0 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}17.1\ssW{}}&
\ssW{}16.9&\ssW{}&
\ssW{}20.5 &\wtC{cbScarlet}{}&
% DTR
\ssW{}21.3 &\wtC{cbScarlet}{} 
\\


Dow & 
%fixpop
\multicolumn{2}{c}{\ssW{}19.9\ssW{}}& 
\ssW{}22.4&\wtC{cbScarlet}{}&
\ssW{}23.9 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}19.1\ssW{}}&
\ssW{}18.7 &\ssW{}&
\ssW{}24.0 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}18.8\ssW{}}&
\ssW{}18.4&\ssW{}&
\ssW{}23.7 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}18.5\ssW{}}&
\ssW{}20.1&\wtC{cbScarlet}{}&
\ssW{}25.2 &\wtC{cbScarlet}{}&
% DTR
\ssW{}27.6 &\wtC{cbScarlet}{} 
\\


EnC & 
%fixpop
\multicolumn{2}{c}{\ssW{}5.3\ssW{}}& 
\ssW{}5.0 &\btC{cbScarlet}{}&
\ssW{}6.9 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}4.4\ssW{}}&
\ssW{}4.8 &\ssW{}&
\ssW{}7.5 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}4.5\ssW{}}&
\ssW{}4.8 &\ssW{}&
\ssW{}9.3 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}4.7\ssW{}}&
\ssW{}4.8 &\wtC{cbScarlet}{}&
\ssW{}8.0 &\wtC{cbScarlet}{} &
% DTR
\ssW{}4.6 &\btC{cbScarlet}{} 
\\


EnH & 
%fixpop
\multicolumn{2}{c}{\ssW{}2.2\ssW{}}& 
\ssW{}1.9 &\btC{cbScarlet}{}&
\ssW{}5.4 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}2.1\ssW{}}&
\ssW{}1.6 &\btC{cbScarlet}{}&
\ssW{}5.3 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}2.1\ssW{}}&
\ssW{}1.8 &\btC{cbScarlet}{}&
\ssW{}5.5 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}2.0\ssW{}}&
\ssW{}1.5 &\ssW{}&
\ssW{}5.8 &\wtC{cbScarlet}{}&
% DTR
\ssW{}0.3 &\btC{cbScarlet}{} 
\\


Tow &
%fixpop
\multicolumn{2}{r}{\ssW{}11.8\ssW{}}& 
\ssW{}13.0 &\wtC{cbScarlet}{}&
\ssW{}18.2 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}11.9\ssW{}}&
\ssW{}12.0&\ssW{}&
\ssW{}18.6 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}11.9\ssW{}}&
\ssW{}12.1 &\ssW{}&
\ssW{}16.7 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}11.8\ssW{}}&
\ssW{}12.0&\ssW{}&
\ssW{}16.9 &\wtC{cbScarlet}{}&
% DTR
\ssW{}11.2 &\btC{cbScarlet}{} 
\\


WiR & 
%fixpop
\multicolumn{2}{r}{\ssW{}61.9\ssW{}}& 
\ssW{}61.6 &\ssW{}&
\ssW{}63.4 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}61.6\ssW{}}&
\ssW{}61.6&\ssW{}&
\ssW{}63.9 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}61.6\ssW{}}&
\ssW{}62.4 &\wtC{cbScarlet}{}&
\ssW{}63.8 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}61.6\ssW{}}&
\ssW{}62.1 &\wtC{cbScarlet}{}&
\ssW{}62.6 &\wtC{cbScarlet}{}&
% DTR
\ssW{}72.0 &\wtC{cbScarlet}{} 
\\


WiW & 
%fixpop
\multicolumn{2}{r}{\ssW{}69.1\ssW{}}& 
\ssW{}69.6 &\wtC{cbScarlet}{}&
\ssW{}70.3 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}69.4\ssW{}}&
\ssW{}69.3 &\ssW{}&
\ssW{}71.1 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}69.3\ssW{}}&
\ssW{}69.5 &\wtC{cbScarlet}{}&
\ssW{}70.6 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}69.7\ssW{}}&
\ssW{}68.9 &\btC{cbScarlet}{}&
\ssW{}70.7 &\wtC{cbScarlet}{}&
% DTR
\ssW{}72.6 &\wtC{cbScarlet}{} 
\\


Yac &
 %fixpop
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}& 
\ssW{}0.4 &\btC{cbScarlet}{}&
\ssW{}0.7 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}&
\ssW{}0.4 &\ssW{}&
\ssW{}0.7 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}&
\ssW{}0.4 &\ssW{}&
\ssW{}0.6 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}&
\ssW{}0.5 &\ssW{}&
\ssW{}0.6 &\wtC{cbScarlet}{}&
% DTR
\ssW{}0.9 &\wtC{cbScarlet}{} 
\\


\midrule

%fixpop
B/W & \multicolumn{2}{c}{---} & \multicolumn{2}{c}{3/6} & \multicolumn{2}{c}{ 0/10 } &
%ims 4
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{2/2} & \multicolumn{2}{c}{0/10} &
%ims 6
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{1/3} & \multicolumn{2}{c}{0/10} &
%ims 8
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{1/4} & \multicolumn{2}{c}{0/10} & \multicolumn{2}{c}{3/7}
\\ 

\bottomrule

\end{tabular}
}
\end{table*}

==> results_test4.tex <==
\begin{table*}
\caption{Median test NMSE with $l \leq 31$, details as in Table~\ref{tab:validation3}.}\label{tab:test}
\centering
\setlength{\tabcolsep}{0.01em}
\scalebox{0.7}{
\begin{tabular}{lScScSccScScSccScScSccScScScSc}
\toprule
 & \multicolumn{6}{c}{$n_\text{pop}=1000$} & \ssW{}\ssW{} & \multicolumn{6}{c}{IMS $g=4$} & \ssW{}\ssW{} & \multicolumn{6}{c}{IMS $g=6$} & \ssW{}\ssW{} & \multicolumn{8}{c}{IMS $g=8$} \\
 
Dataset \ssW{}& \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO}
& \multicolumn{2}{c}{DTR}\\
\midrule

Air & 
%fixpop
\multicolumn{2}{c}{\ssW{}26.4\ssW{}}& 
\ssW{}30.3 &\wtC{cbScarlet}{}&
\ssW{}37.2 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}26.1\ssW{}}&
\ssW{}23.7 &\btC{cbScarlet}{}&
\ssW{}37.4 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}25.1\ssW{}}&
\ssW{}25.3 &\ssW{}&
\ssW{}39.5 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}25.0\ssW{}}&
\ssW{}26.1 &\ssW{}&
\ssW{}39.1 &\wtC{cbScarlet}{}&
% DTR
\ssW{}31.2 &\wtC{cbScarlet}{} 
\\


Bos & 
%fixpop
\multicolumn{2}{c}{\ssW{}20.8\ssW{}}& 
\ssW{}20.9 &\wtC{cbScarlet}{}&
\ssW{}26.4 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}18.8\ssW{}}&
\ssW{}21.3&\wtC{cbScarlet}{}&
\ssW{}22.8&\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}20.4\ssW{}}&
\ssW{}21.5 &\wtC{cbScarlet}{}&
\ssW{}22.7 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}20.0\ssW{}}&
\ssW{}21.4 &\wtC{cbScarlet}{}&
\ssW{}24.4 &\wtC{cbScarlet}{}&
% DTR
\ssW{}25.5 &\wtC{cbScarlet}{} 
\\

Con & 
%fixpop
\multicolumn{2}{c}{\ssW{}17.4\ssW{}}& 
\ssW{}17.7 &\wtC{cbScarlet}{}&
\ssW{}21.6 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}16.9\ssW{}}&
\ssW{}17.1&\wtC{cbScarlet}{}&
\ssW{}21.6 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}16.6\ssW{}}&
\ssW{}16.9&\ssW{}&
\ssW{}21.0 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}17.1\ssW{}}&
\ssW{}16.9&\ssW{}&
\ssW{}20.5 &\wtC{cbScarlet}{}&
% DTR
\ssW{}21.3 &\wtC{cbScarlet}{} 
\\


Dow & 
%fixpop
\multicolumn{2}{c}{\ssW{}19.9\ssW{}}& 
\ssW{}22.4&\wtC{cbScarlet}{}&
\ssW{}23.9 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}19.1\ssW{}}&
\ssW{}18.7 &\ssW{}&
\ssW{}24.0 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}18.8\ssW{}}&
\ssW{}18.4&\ssW{}&
\ssW{}23.7 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}18.5\ssW{}}&
\ssW{}20.1&\wtC{cbScarlet}{}&
\ssW{}25.2 &\wtC{cbScarlet}{}&
% DTR
\ssW{}27.6 &\wtC{cbScarlet}{} 
\\


EnC & 
%fixpop
\multicolumn{2}{c}{\ssW{}5.3\ssW{}}& 
\ssW{}5.0 &\btC{cbScarlet}{}&
\ssW{}6.9 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}4.4\ssW{}}&
\ssW{}4.8 &\ssW{}&
\ssW{}7.5 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}4.5\ssW{}}&
\ssW{}4.8 &\ssW{}&
\ssW{}9.3 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}4.7\ssW{}}&
\ssW{}4.8 &\wtC{cbScarlet}{}&
\ssW{}8.0 &\wtC{cbScarlet}{} &
% DTR
\ssW{}4.6 &\btC{cbScarlet}{} 
\\


EnH & 
%fixpop
\multicolumn{2}{c}{\ssW{}2.2\ssW{}}& 
\ssW{}1.9 &\btC{cbScarlet}{}&
\ssW{}5.4 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}2.1\ssW{}}&
\ssW{}1.6 &\btC{cbScarlet}{}&
\ssW{}5.3 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}2.1\ssW{}}&
\ssW{}1.8 &\btC{cbScarlet}{}&
\ssW{}5.5 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}2.0\ssW{}}&
\ssW{}1.5 &\ssW{}&
\ssW{}5.8 &\wtC{cbScarlet}{}&
% DTR
\ssW{}0.3 &\btC{cbScarlet}{} 
\\


Tow &
%fixpop
\multicolumn{2}{r}{\ssW{}11.8\ssW{}}& 
\ssW{}13.0 &\wtC{cbScarlet}{}&
\ssW{}18.2 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}11.9\ssW{}}&
\ssW{}12.0&\ssW{}&
\ssW{}18.6 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}11.9\ssW{}}&
\ssW{}12.1 &\ssW{}&
\ssW{}16.7 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}11.8\ssW{}}&
\ssW{}12.0&\ssW{}&
\ssW{}16.9 &\wtC{cbScarlet}{}&
% DTR
\ssW{}11.2 &\btC{cbScarlet}{} 
\\


WiR & 
%fixpop
\multicolumn{2}{r}{\ssW{}61.9\ssW{}}& 
\ssW{}61.6 &\ssW{}&
\ssW{}63.4 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}61.6\ssW{}}&
\ssW{}61.6&\ssW{}&
\ssW{}63.9 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}61.6\ssW{}}&
\ssW{}62.4 &\wtC{cbScarlet}{}&
\ssW{}63.8 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}61.6\ssW{}}&
\ssW{}62.1 &\wtC{cbScarlet}{}&
\ssW{}62.6 &\wtC{cbScarlet}{}&
% DTR
\ssW{}72.0 &\wtC{cbScarlet}{} 
\\


WiW & 
%fixpop
\multicolumn{2}{r}{\ssW{}69.1\ssW{}}& 
\ssW{}69.6 &\wtC{cbScarlet}{}&
\ssW{}70.3 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}69.4\ssW{}}&
\ssW{}69.3 &\ssW{}&
\ssW{}71.1 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}69.3\ssW{}}&
\ssW{}69.5 &\wtC{cbScarlet}{}&
\ssW{}70.6 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}69.7\ssW{}}&
\ssW{}68.9 &\btC{cbScarlet}{}&
\ssW{}70.7 &\wtC{cbScarlet}{}&
% DTR
\ssW{}72.6 &\wtC{cbScarlet}{} 
\\


Yac &
 %fixpop
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}& 
\ssW{}0.4 &\btC{cbScarlet}{}&
\ssW{}0.7 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}&
\ssW{}0.4 &\ssW{}&
\ssW{}0.7 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}&
\ssW{}0.4 &\ssW{}&
\ssW{}0.6 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}&
\ssW{}0.5 &\ssW{}&
\ssW{}0.6 &\wtC{cbScarlet}{}&
% DTR
\ssW{}0.9 &\wtC{cbScarlet}{} 
\\


\midrule

%fixpop
B/W & \multicolumn{2}{c}{---} & \multicolumn{2}{c}{3/6} & \multicolumn{2}{c}{ 0/10 } &
%ims 4
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{2/2} & \multicolumn{2}{c}{0/10} &
%ims 6
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{1/3} & \multicolumn{2}{c}{0/10} &
%ims 8
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{1/4} & \multicolumn{2}{c}{0/10} & \multicolumn{2}{c}{3/7}
\\ 

\bottomrule

\end{tabular}
}
\end{table*}

==> results_validation_3.tex <==
\begin{table*}
\caption{Median validation NMSE of 30 runs for GP-GOMEA (GOM), GP-Trad (TRA), GP-RDO (RDO) with $p=1000$ and IMS with $g \in \{ 4, 6, 8 \}$, and DTR. Solution size is limited to 31. Significance is assessed within each population scheme w.r.t. GP-GOMEA. The last row reports the number of times the EA performs significantly better (B) and worse (W) than GP-GOMEA.}\label{tab:validation}
\centering
\setlength{\tabcolsep}{0.01em}
\scalebox{0.7}{
\begin{tabular}{lScScSccScScSccScScSccScScScSc}
\toprule
 & \multicolumn{6}{c}{$p=1000$} & \ssW{}\ssW{} & \multicolumn{6}{c}{IMS $g=4$} & \ssW{}\ssW{} & \multicolumn{6}{c}{IMS $g=6$} & \ssW{}\ssW{} & \multicolumn{8}{c}{IMS $g=8$} \\
 
Dataset \ssW{}& \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & & \multicolumn{2}{c}{\color{cbScarlet}GOM} & \multicolumn{2}{c}{\color{black}TRA} & \multicolumn{2}{c}{\color{black}RDO} & \multicolumn{2}{c}{DTR}\\
\midrule

Air & 
%fixpop
\multicolumn{2}{c}{\ssW{}26.3\ssW{}}& 
\ssW{}32.2 &\wtC{cbScarlet}{}&
\ssW{}35.9 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}34.5\ssW{}}&
\ssW{}31.3 &\btC{cbScarlet}{}&
\ssW{} &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}34.9\ssW{}}&
\ssW{}33.7 &\btC{cbScarlet}{}&
\ssW{} &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}34.3\ssW{}}&
\ssW{}32.7 &\btC{cbScarlet}&
\ssW{} &\wtC{cbScarlet}{} &
% DTR
\ssW{}30.8 &\btC{cbScarlet}{} 
\\


Bos & 
%fixpop
\multicolumn{2}{c}{\ssW{}22.3\ssW{}}& 
\ssW{}19.3 &\ssW{}&
\ssW{}24.0 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}16.7\ssW{}}&
\ssW{}16.0&\wtC{cbScarlet}{}&
\ssW{}19.7&\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}16.5\ssW{}}&
\ssW{}17.1&\wtC{cbScarlet}{}&
\ssW{}20.2 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}17.0\ssW{}}&
\ssW{}17.0 &\wtC{cbScarlet}{}&
\ssW{}20.1 &\wtC{cbScarlet}{}&
% DTR
\ssW{}22.7 &\wtC{cbScarlet}{} 
\\

Con & 
%fixpop
\multicolumn{2}{c}{\ssW{}17.5\ssW{}}& 
\ssW{}18.5 &\wtC{cbScarlet}{}&
\ssW{}21.3 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}16.6\ssW{}}&
\ssW{}17.3&\ssW{}&
\ssW{}20.8 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}17.0\ssW{}}&
\ssW{}17.6&\wtC{cbScarlet}{}&
\ssW{}20.5 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}16.6\ssW{}}&
\ssW{}16.9&\wtC{cbScarlet}{}&
\ssW{}20.4 &\wtC{cbScarlet}{}&
% DTR
\ssW{}22.8 &\wtC{cbScarlet}{} 
\\

Dow & 
%fixpop
\multicolumn{2}{c}{\ssW{}20.9\ssW{}}& 
\ssW{}22.2&\ssW{}&
\ssW{}24.0&\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{c}{\ssW{}19.0\ssW{}}&
\ssW{}19.1 &\ssW{}&
\ssW{}25.6 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}19.4\ssW{}}&
\ssW{}19.9&\wtC{cbScarlet}{}&
\ssW{}25.0 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}19.5\ssW{}}&
\ssW{}19.9&\wtC{cbScarlet}{}&
\ssW{}25.6 &\wtC{cbScarlet}{}&
% DTR
\ssW{}30.6 &\wtC{cbScarlet}{} 
\\

EnC & 
%fixpop
\multicolumn{2}{c}{\ssW{}5.3\ssW{}}& 
\ssW{}5.2 &\btC{cbScarlet}{}&
\ssW{}7.3 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}4.7\ssW{}}&
\ssW{}4.9 &\wtC{cbScarlet}{}&
\ssW{}7.2 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{c}{\ssW{}4.7\ssW{}}&
\ssW{}4.6 &\wtC{cbScarlet}{}&
\ssW{}8.8 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{c}{\ssW{}4.4\ssW{}}&
\ssW{}4.9 &\wtC{cbScarlet}{}&
\ssW{}7.8 &\wtC{cbScarlet}{}&
% DTR
\ssW{}4.1 &\btC{cbScarlet}{} 
\\

EnH & 
%fixpop
\multicolumn{2}{c}{\ssW{}2.3\ssW{}}& 
\ssW{}1.8 &\btC{cbScarlet}{}&
\ssW{}6.0 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}2.0\ssW{}}&
\ssW{}1.5 &\btC{cbScarlet}{}&
\ssW{}5.0 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}2.0\ssW{}}&
\ssW{}1.6 &\btC{cbScarlet}{}&
\ssW{}6.1 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}1.9\ssW{}}&
\ssW{}1.6 &\ssW{}&
\ssW{}5.7 &\wtC{cbScarlet}{}&
% DTR
\ssW{}0.4 &\btC{cbScarlet}{} 
\\

Tow &
%fixpop
\multicolumn{2}{r}{\ssW{}12.0\ssW{}}& 
\ssW{}12.7 &\wtC{cbScarlet}{}&
\ssW{}17.7 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}11.9\ssW{}}&
\ssW{}12.0&\wtC{cbScarlet}{}&
\ssW{}18.2 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}12.1\ssW{}}&
\ssW{}12.2 &\wtC{cbScarlet}{}&
\ssW{}16.6 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}12.0\ssW{}}&
\ssW{}11.9&\wtC{cbScarlet}{}&
\ssW{}17.4 &\wtC{cbScarlet}{}&
% DTR
\ssW{}11.1 &\btC{cbScarlet}{} 
\\

WiR & 
%fixpop
\multicolumn{2}{r}{\ssW{}64.3\ssW{}}& 
\ssW{}64.6 &\ssW{}&
\ssW{}66.0 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}63.2\ssW{}}&
\ssW{}62.8&\ssW{}&
\ssW{}64.5 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}62.8\ssW{}}&
\ssW{}62.9 &\ssW{}&
\ssW{}64.8 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}62.8\ssW{}}&
\ssW{}62.2 &\ssW{}&
\ssW{}64.8 &\wtC{cbScarlet}{}&
% DTR
\ssW{}71.5 &\wtC{cbScarlet}{} 
\\

WiW & 
%fixpop
\multicolumn{2}{r}{\ssW{}70.1\ssW{}}& 
\ssW{}70.2 &\ssW{}&
\ssW{}71.0 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}69.6\ssW{}}&
\ssW{}69.7 &\ssW{}&
\ssW{}70.9 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}69.3\ssW{}}&
\ssW{}69.7 &\ssW{}&
\ssW{}70.4 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}69.8\ssW{}}&
\ssW{}69.3 &\ssW{}&
\ssW{}71.1 &\wtC{cbScarlet}{}&
% DTR
\ssW{}72.2 &\wtC{cbScarlet}{} 
\\

Yac &
%fixpop
\multicolumn{2}{r}{\ssW{}0.5\ssW{}}& 
\ssW{}0.5 &\btC{cbScarlet}{}&
\ssW{}0.6 &\wtC{cbScarlet}{}&
&
%ims 4
\multicolumn{2}{r}{\ssW{}0.4\ssW{}}&
\ssW{}0.4 &\wtC{cbScarlet}{}&
\ssW{}0.6 &\wtC{cbScarlet}{}&
& 
%ims 6
\multicolumn{2}{r}{\ssW{}0.4\ssW{}}&
\ssW{}0.4 &\ssW{}&
\ssW{}0.5 &\wtC{cbScarlet}{}&
&
%ims 8
\multicolumn{2}{r}{\ssW{}0.4\ssW{}}&
\ssW{}0.4 &\wtC{cbScarlet}{}&
\ssW{}0.6 &\wtC{cbScarlet}{}&
% DTR
\ssW{}0.9 &\wtC{cbScarlet}{} 
\\

\midrule

%fixpop
B/W & \multicolumn{2}{c}{---} & \multicolumn{2}{c}{3/3} & \multicolumn{2}{c}{ 0/10 } &
%ims 4
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{2/4} & \multicolumn{2}{c}{0/10} &
%ims 6
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{1/6} & \multicolumn{2}{c}{0/10} &
%ims 8
& \multicolumn{2}{c}{---} & \multicolumn{2}{c}{0/6} & \multicolumn{2}{c}{0/10} & \multicolumn{2}{c}{3/7}
\\ 

\bottomrule

\end{tabular}
}
\end{table*}
